Bridging the Semantic Gap in Virtual Machine Introspection and Forensic Memory Analysis

Forensic Memory Analysis (FMA) and Virtual Machine Introspection (VMI) are critical tools for security in a virtualization-based approach. VMI and FMA involves using digital forensic methods to extract information from the system to identify and explain security incidents. A key challenge in both FMA and VMI is the "Semantic Gap", which is the difficulty of interpreting raw memory data without specialized tools and expertise. In this work, we investigate how a priori knowledge, metadata and engineered features can aid VMI and FMA, leveraging machine learning to automate information extraction and reduce the workload of forensic investigators. We choose OpenSSH as our use case to test different methods to extract high level structures. We also test our method on complete physical memory dumps to showcase the effectiveness of the engineered features. Our features range from basic statistical features to advanced graph-based representations using malloc headers and pointer translations. The training and testing are carried out on public datasets that we compare against already recognized baseline methods. We show that using metadata, we can improve the performance of the algorithm when there is very little training data and also quantify how having more data results in better generalization performance. The final contribution is an open dataset of physical memory dumps, totalling more than 1 TB of different memory state, software environments, main memory capacities and operating system versions. Our methods show that having more metadata boosts performance with all methods obtaining an F1-Score of over 80%. Our research underscores the possibility of using feature engineering and machine learning techniques to bridge the semantic gap.

==> images/machinekex/ssh_struct_tikz.tex <==
\begin{tikzpicture}
	\node[align=center] (function) at (0,0) {kex\_derive\_keys(\textbf{struct ssh *ssh}, ...)};
	
	%struct ssh
	\node[draw, align=center, minimum width=4.2cm, minimum height=0.75cm, pattern=dots] (structssh) at (0,-1.25cm) {\contour{white}{\textbf{struct ssh}}};
	\node[draw, align=center, font=\small, minimum width=4.2cm, minimum height=0.75cm, below=0cm of structssh] (structssh_sessionstate) {struct session\_state *state};
	\node[draw, align=center, font=\small, minimum width=4.2cm, minimum height=0.75cm, below=0cm of structssh_sessionstate] (structssh_kex) {struct kex *kex};
	\node[draw, align=center, font=\small, minimum width=4.2cm, minimum height=0.75cm, below=0cm of structssh_kex] (structssh_others) {...};
	
	%struct session_state
	\node[draw, align=center, minimum width=4.0cm, minimum height=0.75cm, pattern=dots, right=0.75cm of structssh] (structsessionstate) {\contour{white}{\textbf{struct session\_state}}};
	\node[draw, align=center, font=\small, minimum width=4.0cm, minimum height=0.75cm, below=0cm of structsessionstate] (structsessionstate_others1) {...};
	\node[draw, align=center, font=\small, minimum width=4.0cm, minimum height=0.75cm, below=0cm of structsessionstate_others1] (structsessionstate_newkeys) {struct newkeys *newkeys[]};
	\node[draw, align=center, font=\small, minimum width=4.0cm, minimum height=0.75cm, below=0cm of structsessionstate_newkeys] (structsessionstate_others2) {...};
	
	%struct newkeys
	\node[draw, align=center, minimum width=2.95cm, minimum height=0.75cm, pattern=dots, right=0.75cm of structsessionstate] (structnewkeys) {\contour{white}{\textbf{struct newkeys}}};
	\node[draw, align=center, font=\small, minimum width=2.95cm, minimum height=0.75cm, below=0cm of structnewkeys] (structnewkeys_structsshenc) {struct sshenc enc};
	\node[draw, align=center, font=\small, minimum width=2.95cm, minimum height=0.75cm, below=0cm of structnewkeys_structsshenc] (structnewkeys_structsshmac) {struct sshmac mac};
	\node[draw, align=center, font=\small, minimum width=2.95cm, minimum height=0.75cm, below=0cm of structnewkeys_structsshmac] (structnewkeys_structscomp) {struct comp comp};
	
	%struct sshenc
	\node[draw, align=center, minimum width=2.75cm, minimum height=0.75cm, pattern=dots, right=0.75cm of structnewkeys] (structsshenc) {\contour{white}{\textbf{struct sshenc}}};
	\node[draw, align=center, font=\small, minimum width=2.75cm, minimum height=0.75cm, below=0cm of structsshenc] (keylen) {u\_int key\_len};
	\node[draw, align=center, font=\small, minimum width=2.75cm, minimum height=0.75cm, below=0cm of keylen] (ivlen) {u\_int iv\_len};
	\node[draw, align=center, font=\small, minimum width=2.75cm, minimum height=0.75cm, below=0cm of ivlen] (keypoint) {u\_char *key};
	\node[draw, align=center, font=\small, minimum width=2.75cm, minimum height=0.75cm, below=0cm of keypoint] (ivpoint) {u\_char *iv};
	\node[draw, align=center, font=\small, minimum width=2.75cm, minimum height=0.75cm, below=0cm of ivpoint] (structsshenc_others) {...};
	
	%key and iv
	\node[draw, align=center, font=\small, minimum width=1cm, minimum height=0.75cm, right=0.5cm of keypoint, yshift=0.25cm] (key) {Key};
	\node[draw, align=center, font=\small, minimum width=1cm, minimum height=0.75cm, right=0.5cm of ivpoint, yshift=-0.25cm] (iv) {IV};
	
	%lines
	\draw [>=stealth, very thick, ->] ([xshift=0.75cm]function.south) -- ([yshift=-0.5cm,xshift=0.75cm]function.south);
	\draw [>=stealth, very thick, ->] (structssh_sessionstate.east) -| ([xshift=0.375cm]structssh_sessionstate.east) -- ([xshift=-0.345cm]structsessionstate.west) |- (structsessionstate.west);
	\draw [>=stealth, very thick, ->] (structsessionstate_newkeys.east) -| ([xshift=0.335cm]structsessionstate_newkeys.east) -- ([xshift=-0.375cm]structnewkeys.west) |- (structnewkeys.west);
	\draw [>=stealth, very thick, ->, dashed] (structnewkeys_structsshenc.east) -| ([xshift=0.375cm]structnewkeys_structsshenc.east) -- ([xshift=-0.375cm]structsshenc.west) |- (structsshenc.west);
	\draw [>=stealth, very thick, ->] (keypoint) -- (key);
	\draw [>=stealth, very thick, ->] (ivpoint) -- (iv);
	
\end{tikzpicture}
